Deriving Abstract Interpreters from Skeletal Semantics

This paper describes a methodology for defining an executable abstract interpreter from a formal description of the semantics of a programming language. Our approach is based on Skeletal Semantics and an abstract interpretation of its semantic meta-language. The correctness of the derived abstract interpretation can be established by compositionality provided that correctness properties of the core language-specific constructs are established. We illustrate the genericness of our method by defining a Value Analysis for a small imperative language based on its skeletal semantics.

==> eptcsdata.tex <==
\providecommand{\firstpage}{97}
\providecommand{\publicationstatus}{G. Caltais and C. A. Mezzina (Eds): Combined Workshop on\\
Expressiveness in Concurrency and Structural Operational Semantics\\(EXPRESS/SOS 2023).\\
EPTCS 387, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.387.8}{10.4204/EPTCS.387.8}}

